UnifiedSKG: Unifying and Multi-Tasking Structured Knowledge Grounding with Text-to-Text Language Models

Structured knowledge grounding (SKG) leverages structured knowledge to complete user requests, such as semantic parsing over databases and question answering over knowledge bases. Since the inputs and outputs of SKG tasks are heterogeneous, they have been studied separately by different communities, which limits systematic and compatible research on SKG. In this paper, we overcome this limitation by proposing the UnifiedSKG framework, which unifies 21 SKG tasks into a text-to-text format, aiming to promote systematic SKG research, instead of being exclusive to a single task, domain, or dataset. We use UnifiedSKG to benchmark T5 with different sizes and show that T5, with simple modifications when necessary, achieves state-of-the-art performance on almost all of the 21 tasks. We further demonstrate that multi-task prefix-tuning improves the performance on most tasks, largely improving the overall performance. UnifiedSKG also facilitates the investigation of zero-shot and few-shot learning, and we show that T0, GPT-3, and Codex struggle in zero-shot and few-shot learning for SKG. We also use UnifiedSKG to conduct a series of controlled experiments on structured knowledge encoding variants across SKG tasks. UnifiedSKG is easily extensible to more tasks, and it is open-sourced at https://github.com/hkunlp/unifiedskg.

==> tables/curves.tex <==
\begin{figure}[ht]
    \centering
	\includegraphics[scale=0.4]{./figures/length/length_distribution_and_perform_effect.pdf}
	\caption{Learning curves of selected tasks.}
	\label{fig:length-effect-wikitq}
\end{figure}

==> tables/multi_task_all_tasks.tex <==
\begin{table*}[ht]
	\centering
	\begin{adjustbox}{width=\linewidth}
		\begin{tabular}{@{}lccccccc@{}}
			\toprule
			& Metric & T5-base & T5-base (prefix) & T5-base (pretrained prefix) & T5-base (stage-3) 
			& T5-large
			& T5-3B
			\\ 
			\midrule
			%\multicolumn{6}{c}{\textit{Semantic Parsing}} \\
			%\midrule
	        \multirow{3}*{Spider} 
            & Match & 58.12 & 58.61 & & & 68.38 & 71.5 \\
            & Exec & 59.57 & 60.35 & & & 70.02 & 74.4 \\
            & Test suite & 56.22 & 64.12 & & & -- & -- \\
            \midrule
            \multirow{1}*{GrailQA}
            & Match & 60.00 & 63.33 & & & 67.00 & 69.00 \\
            \midrule
            \multirow{1}*{WebQSP}
            & F1 & 72.50 & 73.81 & & & 73.96 & 75.97 \\
            \midrule
            \multirow{1}*{MTOP}
            & Match & 83.89 & 82.93 & & & 84.70 & 84.88 \\
			\midrule
			%\multicolumn{6}{c}{\textit{Question Answering}} \\
			%\midrule
            \multirow{1}*{WikiTQ}
            & Acc & 36.94 & 36.42 & 39.74 & & 43.30 & 50.65 \\
            \midrule
            \multirow{1}*{WikiSQL}
            & Acc & 84.50 & 83.09 &  & & 86.27 & 87.34 \\
            \midrule
            \multirow{1}*{CompWebQ}
            & Acc & 66.71 & 67.85 & & & 69.42 & 70.27 \\
            %& F1 & 80.02 & 80.14 & & & 81.05 & 81.43 \\
            \midrule
            \multirow{1}*{HybridQA}
            & Acc & 54.07 & 54.93 & & & 56.96 & 58.92 \\
            %& F1 & 61.85 & 62.35 & & & 64.62 & 66.29 \\
            \midrule
            \multirow{2}*{MMQA}
            & Acc & 67.29 & 67.62 & & & 74.08 & 78.48 \\
            & F1 & 75.51 & 75.50 & & & 81.84 & 82.28 \\
            \midrule
            \multirow{1}*{FeTaQA}
            & BLEU & 29.12 & 28.03 & 29.33 & & 30.94 & 33.44 \\
			\midrule 
			%\multicolumn{6}{c}{\textit{Data-to-text}} \\
			%\midrule
			\multirow{1}*{DART} 
			& BLEU & 50.62 & 50.33 & & & 51.72 & 50.38 \\
            \midrule
			\multirow{1}*{ToTTo}
			& BLEU & 48.29 & 45.70 & & & 48.95 & 48.95 \\
			%& BLEURT & \running & 32.00 & \running \\
            \midrule
			%\multicolumn{6}{c}{\textit{Conversational}} \\
			%\midrule 
			\multirow{1}*{MultiWoZ2.1}
			& Joint Acc & 57.52 & 56.67 & & & 58.23 & 58.46 \\
            \midrule
			\multirow{1}*{KVRET}
			& BLEU & 20.04 & 19.68 & 21.32 & & 18.84 & 17.75 \\
            \midrule
			\multirow{1}*{SParC}
			& Match & 50.54 & 52.54 & & & 56.69 & 61.51 \\
			%& Exec & 53.95 & 55.28 & & & 60.60 & 67.33 \\
			%& Match (interact) & 27.96 & 29.15 & & & 35.55 & 40.05 \\
			%& Exec (interact) & 31.26 & 32.46 & & & 38.39 & 44.08 \\
			\midrule
			\multirow{1}*{CoSQL}
			& Match & 42.30 & 44.39 & 45.68 & & 48.26 & 53.8 \\
			%& Match (interact) & 7.85 & 10.58 & & & 12.29 & 21.8 \\
			%& Exec & 49.26 & 52.43 & 51.54 & & 56.01 & -- \\
			%& Exec (interact) & 10.85 & 15.36 & & & 15.36 & -- \\
			\midrule
			\multirow{1}*{SQA}
			& Overall Acc & 49.49 & 44.81 & & & 59.12 & 60.93 \\
			%& Pos 0 Acc  & 57.65 & 46.68 & & & 63.65 & 59.18 \\
			%& Pos 1 Acc  & 47.96 & 44.77 & & & 57.02 & 61.73 \\
			%& Pos 2 Acc  & 43.27 & 43.27 & & & 56.73 & 62.57 \\
			%& Pos 3 Acc  & 40.52 & 41.18 & & & 55.56 & 61.44 \\
			\midrule
			\multirow{1}*{TabFact}
			& Acc & 76.34 & 75.74 & & & 81.40 & 83.97 \\
			\midrule
            \multirow{1}*{FEVEROUS}
            & Acc & 75.05 & 75.33 & & & 79.81 & 82.40 \\
			\midrule
			\multirow{1}*{SQL2Text}
			& BLEC & 93.43 & 94.50 & 93.79 & & 93.07 & 92.71 \\
            \midrule
			\multirow{1}*{Logic2Text}
			& BLEC & 92.15 & 95.25 & & & 92.88 & 91.69 \\
			\bottomrule
		\end{tabular}
		\end{adjustbox}
	\caption{Development set performance of prefix-augmented multi-task learning. }
	\label{tab:multitask-dev}
\end{table*}

\begin{table*}[ht]
	\centering
	\begin{adjustbox}{width=\linewidth}
		\begin{tabular}{@{}lccccccc@{}}
			\toprule
			& Metric & T5-base & T5-base (stage-1) & T5-base (stage-2) & T5-base (stage-3)
			& T5-large
			& T5-3B 
			\\ 
			\midrule
            \multirow{1}*{GrailQA}
            & Match & 62.39 & 63.92 & & & 67.30 & 70.11 \\
            \midrule
            \multirow{1}*{WebQSP}
            & F1 & 78.83 & 75.77 & & & 79.45 & 80.70 \\
			\midrule
			\multirow{1}*{MTOP}
            & Match & 85.49 & 84.58 & & & 86.17 & 86.78 \\
			\midrule
			%\multicolumn{6}{c}{\textit{Question Answering}} \\
			%\midrule
            \multirow{1}*{WikiTQ}
            & Acc & 35.76 & 35.36 & 38.14 & & 43.16 & 49.29  \\
            \midrule
            \multirow{1}*{WikiSQL}
            & Acc & 82.63 & 81.37 & & & 84.80 & 85.96 \\
            \midrule
            \multirow{2}*{CompWebQ}
            & Acc & 68.43 & 68.75 & & & 71.38 & 73.26 \\
            & F1 & 80.20 & 79.35 & & & 81.76 & 82.58 \\
            \midrule
            %\multirow{2}*{HybridQA}
            %\midrule
            %\multirow{2}*{OTT-QA}
            %\midrule
            %\multirow{2}*{MMQA}
            %\midrule
            \multirow{1}*{FeTaQA}
            & BLEU & 29.95 & & & & 32.45 & 33.44 \\
			\midrule 
			%\multicolumn{6}{c}{\textit{Data-to-text}} \\
			%\midrule
			\multirow{1}*{DART} 
            & BLEU & 46.22 & & & & 47.83 & 47.61 \\
            %& TER & 61.80 & & & & \running & \running \\
            %& METEOR & 55.09 & & & & \running & \running \\
            %& BertScore-F1 & 95 & & & & \running & \running \\
            %& BLEURT & 28.33 & & & & \running & \running \\
            \midrule
			%\multirow{2}*{ToTTo}
            %\midrule
			%\multicolumn{6}{c}{\textit{Conversational}} \\
			%\midrule 
			\multirow{1}*{MultiWoZ2.1}
            & Joint Acc & 54.64 & 52.96 & & & 54.45 & 55.42 \\
            \midrule
			\multirow{2}*{KVRET}
            & BLEU & 17.41 & 18.61 & & & 17.27 & 15.45 \\
            & Overall F1 & 67.21 & 67.73 & & & 68.91 & 70.30 \\
            \midrule
			\multirow{1}*{SQA}
            & Overall Acc  & 52.91 & 47.69 & & & 61.28 & 62.37 \\
            %& Pos 0 Acc  & 62.93 & 52.39 & & & 67.80 & 59.51 \\
            %& Pos 1 Acc  & 44.43 & 41.70 & & & 55.08 & 60.25 \\
            %& Pos 2 Acc  & 50.44 & 48.39 & & & 61.88 & 68.77 \\
            %& Pos 3 Acc  & 53.71 & 50.66 & & & 58.08 & 65.07 \\
			\midrule
			%\multicolumn{6}{c}{\textit{Fact Verification}} \\
			%\midrule
			\multirow{1}*{TabFact}
            & Acc & 76.12 & 76.05 & & & 80.85 & 83.68 \\
            \midrule
            %\multirow{2}*{FEVEROUS} 
            %& Acc & - & - & - \\
			%\midrule
			\multirow{1}*{SQL2Text}
            & BLEC & 92.94 & 92.84 & & & 94.97 & 94.78 \\
            \midrule
			\multirow{1}*{Logic2Text}
            & BLEC & 90.66 & 91.76 & & & 90.57 & 91.39 \\
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption{Test set performance of prefix-augmented multi-task learning (for tasks with a publicly available test set). }
	\label{tab:multitask-test}
\end{table*}

==> tables/multitask_old.tex <==
\begin{table}[ht]
	\centering
	\begin{adjustbox}{width=\columnwidth}
		\begin{tabular}{ccccc}
			\toprule
			Task A & Task B & Type & B only & A to B \\
			\midrule 
	        \multirow{1}*{Spider}
	        & \multirow{1}*{CoSQL}
	        & \multirow{1}*{similar} 
	        &  & 48.26   \\
			\multirow{1}*{Spider}
			& \multirow{1}*{GrailQA}
	        & parallel & 67.00 & 67.00 \\
			\multirow{1}*{Spider}
			& \multirow{1}*{WikiTQ}
            & subtask & 43.40 & 41.68 \\
			\multirow{1}*{SQL2Text}
			& \multirow{1}*{Spider}
			& \multirow{1}*{inverse} 
			& 64.73 & 62.57 \\
			\multirow{1}*{WikiSQL}
			& \multirow{1}*{TabFact}
			& related & 81.40 & 82.76 \\
			\multirow{1}*{TabFact}
			& \multirow{1}*{WikiTQ}
			& related & 43.30 & 45.88 \\
			\multirow{1}*{Spider}
			& \multirow{1}*{TabFact}
			& related & 81.40 & 80.39 \\
			\multirow{1}*{WikiSQL}
			& \multirow{1}*{FeTaQA}
	        & sim in & 30.94 & 31.19 \\
			\multirow{1}*{Logic2Text}
			& \multirow{1}*{SQL2Text}
			& sim out & 93.07 &  \\
	        \bottomrule
		\end{tabular}
		\end{adjustbox}
	\caption{Task relationship analysis on T5-large. \textit{B only} means training the model on task B; \textit{A to B} means training the model on task A and then finetuning the model on task B. In both settings, we report task B's performance. }
	\label{tab:task-relationship-old}
\end{table}

==> tables/skgpretrain.tex <==
\begin{table*}[ht]
	\centering
	\small
	\begin{adjustbox}{width=0.98\linewidth}
		\begin{tabular}{@{}l@{}cc@{}}
			\toprule
			& Metric  T5-3B & SOTA (w/ extra data)
			\\ 
			\midrule
			%\multicolumn{7}{c}{\textit{Semantic Parsing}} \\
			%\midrule
	        \multirow{1}*{Spider (dev)} 
            & Match & 71.50 & 74.7 \cite{rubin-berant-2021-smbop} \\
			\midrule
            \multirow{1}*{WikiTQ}
            & Acc & 49.29 & 57.5 \cite{liu2021tapex}\\
            \multirow{1}*{WikiSQL}
            & Acc & 85.96 & 89.5 \cite{liu2021tapex}\\
            \multirow{1}*{HybridQA (dev)}
            & Acc & 66.29 & 63.4 \cite{eisenschlos2021mate} \\
            \multirow{1}*{MMQA (dev)}
            & Acc & 85.28 & 83.8 \cite{yoran2021turning} \\
			\multirow{1}*{DART}
			& BLEU & 46.22$_{0.66}$ & \textbf{47.83}$_{0.59}$ & 47.61 & 47.2 \cite{aghajanyan2021htlm} \\
            \midrule
			\multirow{1}*{MultiWoZ2.1}
			& Joint Acc & 55.42 & 60.48 \cite{yu2021SCoRE}\\
			\multirow{1}*{SParC (dev)}
			& Match & 61.51 & 62.4 \cite{yu2021SCoRE}\\
			\multirow{1}*{CoSQL (dev)}
			& Match & 53.80 & 52.1 \cite{yu2021SCoRE}\\
			\multirow{1}*{SQA}
			& Overall Acc  & 62.37 & 74.5 \cite{liu2021tapex}\\
			\midrule
			\multirow{1}*{TabFact}
			& Acc & 76.13$_{0.39}$ & 80.85$_{0.24}$ & \bf 83.68 & 74.4 \cite{yang-etal-2020-program} & 84.2 \cite{liu2021tapex}\\
			\midrule
			\bottomrule
		\end{tabular}
	\end{adjustbox}
	\caption{Comparison in performance of T5-3B and SOTA with model further pretrained on structured knowledge data. 
	} 
	\label{tab:skg_pretrain}
\end{table*}

